Statistical Learning under Heterogeneous Distribution Shift

This paper studies the prediction of a target $\mathbf{z}$ from a pair of random variables $(\mathbf{x},\mathbf{y})$, where the ground-truth predictor is additive $\mathbb{E}[\mathbf{z} \mid \mathbf{x},\mathbf{y}] = f_\star(\mathbf{x}) +g_{\star}(\mathbf{y})$. We study the performance of empirical risk minimization (ERM) over functions $f+g$, $f \in F$ and $g \in G$, fit on a given training distribution, but evaluated on a test distribution which exhibits covariate shift. We show that, when the class $F$ is "simpler" than $G$ (measured, e.g., in terms of its metric entropy), our predictor is more resilient to heterogeneous covariate shifts} in which the shift in $\mathbf{x}$ is much greater than that in $\mathbf{y}$. Our analysis proceeds by demonstrating that ERM behaves qualitatively similarly to orthogonal machine learning: the rate at which ERM recovers the $f$-component of the predictor has only a lower-order dependence on the complexity of the class $G$, adjusted for partial non-indentifiability introduced by the additive structure. These results rely on a novel H\"older style inequality for the Dudley integral which may be of independent interest. Moreover, we corroborate our theoretical findings with experiments demonstrating improved resilience to shifts in "simpler" features across numerous domains.

==> body/body_simple.tex <==
%!TEX root = ../main_simple.tex
\newcommand{\genn}{\mathrm{gen}_n}
\newcommand{\ghat}{\hat{g}}
\newcommand{\gst}{g^\star}

\section{Simple Write Up}

\paragraph{Basic setup.}
We consider empirical risk minimization over a function class with an additive decomposition. Let $P_0$ be a distribution over $(\cX,\cY,\cZ)$ where $\cZ \subset \RR$ is a label space and $(\cX,\cY)$ is the instance space. We consider a function class $\cH = \{ f + g : f \in \cF, g \in \cG \} \subset (\cX\times\cY \to \cZ)$ where $\cF \subset \cX \to \cZ$ and $\cG \subset \cY \to \cZ$ are function classes for each component of the input. 

Let $P_1$ be another distribution over $(\cX,\cY,\cZ)$. We
ultimately care about prediction performance on $P_1$ but we only have
samples from $P_0$ for training. To facilitate this transfer we assume
realizability and covariate shift:

\begin{assumption}
  \label{assum:realizability}
  We assume that $\forall x,y: z \mid x,y \sim \cN(f^\star(x) +
  g^\star(y), \sigma^2)$ under both $P_0$ and $P_1$, where $f^\star
  \in \cF$ and $g^\star \in \cG$. 

  %Additionally we assume that $f+g \in [-B,B]$ for all $(f,g) \in \cF \times \cG$.
\end{assumption}

Based on this, for $b \in \{0,1\}$ the population regret is defined as
\begin{align*}
    R_b(h) = R_b(f,g) = \Exp_b\sbr{ ( f(x) + g(y) - f^\star(x) - g^\star(x))^2 } 
\end{align*}

\paragraph{Algorithm.}
We consider ERM over $n$ iid samples from $P_0$. Specifically, we have $\{(x_i,y_i,z_i)\}_{i=1}^n$ drawn iid from $P_0$ and we define:
\begin{align}
    (\hat{f},\hat{g}) = \argmin_{f \in \cF, g \in \cG} \hat{R}_n(f,g), \textrm{ where } \hat{R}_n(f,g) := \frac{1}{n} \sum_{i=1}^n (f(x_i) + g(y_i) - z_i)^2. \label{eq:joint_train}
\end{align}
Our goal is to show that $R_1(\hat{f},\hat{g})$ is small. 

\subsection{The style of our guarantee.}
Informally, our results show that when $\cF$ is simple, we may be more robust to shifts in the distribution of $x$ than those of $y$. To formalize this, suppose we have upper bounds on the distribution shift
\begin{align*}
\sup_{x,y}\frac{\rmd P_1(x,y)}{\rmd P_0(x,y)} \le \kappa_{x,y} , \quad \sup_{y}\frac{\rmd P_1(y)}{\rmd P_0(y)} \le \kappa_{y} 
\end{align*}
Moreover, suppose that $\genn(\cF)$ captures the expected generalization error one would expect if one trained $\fhat$ alone on $P_0$ from labels $\fst(x_i)$:
\begin{align*}
\genn(\cF) \ge \Exp_{P_0}[(\fhat(x) - \fst(x))^2], \quad \fhat \in \argmin_{f \in \cF}\sum_{i=1}^n (f(x_i) - \fst(x_i) - w_i)^2, \quad x_i \iidsim P_0, ~w_i \iidsim \cN(0,\sigma^2)
\end{align*} 
Similarly, suppose $\genn(\cG)$ captures the generalization error of training $\ghat$ in a similar fashion:
\begin{align*}
\genn(\cG) \ge \Exp_{P_0}[(\ghat(y) - \gst(y))^2], \quad \ghat \in \argmin_{g \in \cG}\sum_{i=1}^n (g(y_i) - \gst(y_i) -w_i)^2, \quad y_i \iidsim P_0, ~w_i \iidsim \cN(0,\sigma^2)
\end{align*} 

\paragraph{Naive Bound.} It is standard to show that, for $\hat f, \hat g$ trained in \Cref{eq:joint_train}, the in-distribution generalization is more or less additive
\begin{align*}
R_0(\hat{f},\hat{g}) \lesssim \genn(\cF) + \genn(\cG)
\end{align*}
Hence, a naive change-of-distribution argument leads to the following out-of-distribution error bound
\begin{align}
R_1(\hat{f},\hat{g}) \lesssim \kappa_{x,y}\left(\genn(\cF) + \genn(\cG)\right). \label{eq:naive}
\end{align}

\paragraph{Our bound.} What we are able to show, under mild conditions, is the that \Cref{eq:naive} can be improved to 
\begin{align}
R_1(\hat{f},\hat{g}) \lesssim \kappa_{x,y}\left(\genn(\cF) + o(\genn(\cG))\right) + \kappa_{y}\genn(\cG) \label{eq:better},
\end{align}
where $o(\genn(\cG))$ is a term typically of much lower order than $\genn(\cG)$, and in some cases, is neglible. When this term is neglibile, or at least, dominated by $\genn(\cF)$, we obtain 
\begin{align}
R_1(\hat{f},\hat{g}) \lesssim \kappa_{x,y} \genn(\cF) +  \kappa_{y}\genn(\cG) 
\end{align}
In particular, when $\genn(\cG) \gg \genn(\cF)$, which happens when $\cF$ is much ``simpler'' than $\cG$, we have much greater resilience to covariate shifts in the $x$ variable than in the $y$.

\section{Experiment notes}

\begin{itemize}
  \item It would be cool to have a synthetic setup where our
    performance after distribution shift with decomposable classifier
    is comparable to the in-distribution performance of a
    non-decomposable classifier. For our theory to work (specifically
    realizability), this would require the tasks to be
    different. Perhaps here is one attempt. Let the simple task be
    gray-scale MNIST where your goal is to predict even and odd. The
    more complicated task is colorized MNIST where colors are red/blue
    and this is chosen independently of the image. The task here is to
    predict label $1$ if the image is ``blue and even or odd and red''
    and to predict zero otherwise. Say in the original distribution we
    see red/blue with 50/50 probability but then we shift only the
    color to see red/blue with 75/25 probability (again independent of
    the shape). Is the performance here ``bottlenecked'' by the
    ability to recognize even and odd digits?
\end{itemize}

==> body/classical_examples.tex <==
%!TEX root = ../main.tex
\section{Classical Examples}
\subsection{Linear Regression}
Consider linear regression with $y_i = \langle \bx_i, \bstw \rangle + \xi_i$, where $\xi_i$ are $1$-subGaussian random vectors, and $\bx_i$ are subgaussian with $\Exp[\bx_i\bx_i^\top] = \Sigzero$. 
\begin{proposition} With probabiltity at least $1 - \delta - \exp(-\Omega(n))$, it holds that 
\begin{align*}
\Renv(\what) \lesssim \frac{1}{n}\left(\trace(\Sigenv \Sigzero^{-1} ) + \fronorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}}\log^{1/2}(1/\delta) + \opnorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}} \log(1/\delta)\right).
\end{align*}
\end{proposition}
\begin{proof}
Then, for any $\bhatw$, one 
\begin{align*}
\Renv(\what) = \what^\top \Sigenv \what = \bxi^\top \bX^{\dagger} \Sigenv \bX^{\dagger} \bxi,
\end{align*}
where above $\bxi = (\xi_1,\dots,\xi_n)$, and $\bX$ is a matrix whose rows are $\bx_i \in \R^n$.
By the Hanson-Wright inequality, we have that for $\bZ = \bX^{\top \dagger}\Sigenv \bX^\dagger$
\begin{align*}
\Renv(\what) = \bxi^\top \bX^{\dagger} \Sigenv \bX^{\dagger} \bxi \lesssim \trace(\bZ) + \fronorm{\bZ}\log^{1/2}(1/\delta) + \opnorm{\bZ} \log(1/\delta).
\end{align*}
Using that, for any Schattern $p$-norm $\|\cdot\|$, we have $\|\bA\bA^\top\| = \|\bA^\top\bA\|$, the above inequality holds as well for $\bZ' = \Sigenv^{1/2} \bX^{\dagger} \bX^{\dagger \top} \Sigenv^{1/2} = \Sigenv^{1/2} ( \bX^\top \bX)^{-1} \Sigenv^{1/2}$, provided that $\bX^\top \bX$ is invertible.

Now, using that for $n \ge \tilde{\Omega}(d)$, we have that $\bX^\top \bX \succeq \frac{n}{2}\Sigzero$. Hence, on this event, $(\bX^\top \bX)^{-1} \preceq 2\Sigzero^{-1}/2$. Thus, we have 
\begin{align*}
\Renv(\what) &\lesssim \frac{1}{n}\left(\trace(\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}) + \fronorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}}\log^{1/2}(1/\delta) + \opnorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}} \log(1/\delta)\right)\\
&= \frac{1}{n}\left(\trace(\Sigenv \Sigzero^{-1} ) + \fronorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}}\log^{1/2}(1/\delta) + \opnorm{\Sigenv^{1/2} \Sigzero^{-1} \Sigenv^{1/2}} \log(1/\delta)\right).
\end{align*}
\end{proof}
\subsection{Classification}
\newcommand{\lzone}{\ell_{01}}
\newcommand{\Rzone}{\cR_{01}}
We consider the following stylized classification setting, in the under-parametrized regime where we minimize the $0$-$1$ loss. We assume that there exists some $\wst$ such that
\begin{align*}
\forall \env \in \envs, \quad \Prenv[ y\langle \bx, \wst \rangle \ne 1] \le \eta, \quad \eta \in (0,1/2), \quad \bx \sim \cN(0,\Sigenv), 
\end{align*}
We consider all proper classifers which minimize the zero-one loss $\lzone(\what;\bx,y) := \I\{y\langle \bx,\what\rangle \ne 0\}$ .We may assume without loss of generality that $\wst$ and $\what$ are unit vectors. For this loss,
\begin{lemma}\label{lem:class_error_formula} There exist a universal constant $c > 0$ such that the following holds. Suppose that the marginal distribution of $\bx$ under $\Prenv$ is $\Sigenv^{1/2} \bz$, where $\bz$ has any spherically-symetric distribution on any dimension $d$. Then, defining $\bstv := \Sigenv^{-1/2} \bwst/\|\Sigenv^{-1/2} \bwst\|$  and $\bhatv := \Sigenv^{-1/2}\bhatw/\|\Sigenv^{-1/2} \bhatw\|$,
\begin{align*}
\Renv(\what) \le c \|\Sigenv^{-1/2} \bstw\|^{-1} \cdot \min_{\gamma \ge 0}\|\Sigenv^{-1/2}(\bstw - \gamma \bhatw)\|. 
\end{align*}
\end{lemma}

\begin{comment}Next, we study the structure of the error of $\what$ trained on samples from $\Sigzero$. Note that by a change of basis, we may assume $\Sigzero = \eye_d$, remembering to convert $\Sigenv$ to $\Sigzero^{-1/2}\Sigenv \Sigzero^{-1/2}$ at the end of the proof.
\newcommand{\subj}[1][j]{_{(#1)}}
\newcommand{\subjc}[1][j]{_{(#1)^c}}
Let $\bv_1,\dots,\bv_d$ denote the eigenvectors of $\Sigenv$, and let $\cI_1,\dots,\cI_m$ denote a partition of $[d]$ into non-empty intervals of integers $\cI_j$ such that, for each $j$,  $\lambda_a(\Sigenv) \le 2\lambda_b (\Sigenv)$, where $a = \argmin(\cI_j)$ and $b = \argmax(\cI_j)$, and set $\lambda\subj = \lambda_a$ for that same $a$. For vectors $\bw$, let $\bw\subj$ denote the orthogonal projection of $\bw$ onto $\mathrm{span}(\bv_i, ~i \in \cI_j)$. Lastly, set $M_j = |\cI_j|$. Then, we have
\begin{align*}
\Renv(\what) \le c \|\Sigenv^{-1/2} \bstw\|^{-1} \cdot \min_{\gamma \ge 0}\sum_{j=1}^m \lambda\subj^{1/2}\cdot \|\bstw\subj - \gamma \bhatw_{(0)]}\|
\end{align*}
\end{comment}
Let us now analyze the errors. We shall make two assumptions:
\newcommand{\alg}{\mathsf{alg}}
\newcommand{\GL}{\mathbb{GL}}
We define the $\Sigzero$-weighted orthogonal group as follows:
\begin{align*}
\bbO(\Sigzero) := \{\bO \in \GL(d): \bO^\top \Sigzero^{-1} \bO = \Sigzero^{-1}\}
\end{align*}
\begin{assumption}\label{asm:alg_equivariant} Our algorithm is rotationally equivariant. That is, for any orthgonal matrix $\bO \in \bbO(\Sigzero)$, the distribution of $\bO \cdot \alg((\bx_{i},y_i)_{i \in [n]})$, where $(\bx_i,y_i) \iidsim \Pzero$ is the same as the distribution of $\alg((\bO\cdot\bx_{i},y_i)_{i \in [n]})$ 
\end{assumption}
The second assumption is on the generative distribution:
\begin{assumption}\label{asm:label_invariant} Fix $\bstw$. Then, under $\Pzero$, $\Pzero[y_i \in \cdot \mid \bx] = \Pzero[y_i \mid \langle \bx, \Sigzero^{-\half}\bstw \rangle, ~ \|\bx\|_{\Sigzero^{-1}}^2]$. In other words, the dstribution over labels is invariant under elements of $\bbO(\Sigzero)$ which fix $\Sigzero^{-1/2}\bstw$. 
\end{assumption}
The key object we analyze is $\bhatw^{\perp}$, defined by
\begin{align*}
\bhatw^{\perp} := (\eye_d - \bP_{\envzero}) \Sigzero^{-\half} \bhatw, \quad \bP_{\envzero} :=   \frac{\Sigzero^{-1/2}\bstw (\Sigzero^{-1/2}\bstw)^\top}{\|\Sigzero^{-1/2}\bstw\|^2}
\end{align*}
\begin{lemma} Define \Cref{asm:label_invariant,asm:alg_equivariant}, $\bhatw^{\perp}$ is distributed uniformly on the $d-2$-sphere defined by $\cS_{\envzero} := \{\bw:\|\bw\| = 1, \quad \langle \bw, \Sigzero^{-1/2}\bstw \rangle = 0\}$
\end{lemma}

\begin{theorem}\label{thm:dist_shift_class} Suppose that $\alpha_{\star} := \cos(\theta(\Sigzero^{-\half}\bstw,\Sigzero^{-\half}\bhatw)) > 0 $. Then, with high probability, 
\begin{align*}
\Renv(\what) \lesssim \frac{ 1}{\alpha_{\star}\|\Sigenv^{-\half} \bstw\|} \sqrt{\trace(\Sigenv^{-1}\Sigzero^{\half}(\eye_d - \bP_{\envzero})\Sigzero^{\half} )} + \text{(lower order.)},
\end{align*}
\end{theorem}



We need a lower bound on the risk:






\subsection{Omitted Proofs}
\begin{proof}[Proof of \Cref{lem:class_error_formula}] Since sign-classifiers are positive homogenous, we may assume without loss of generality that $\bz \sim \cN(0,\eye_d)$.
Introduce $\bstv := \Sigenv^{-1/2} \bwst/\|\Sigenv^{-1/2} \bwst\|$ and $\bhatv := \Sigenv^{-1/2}\bhatw/\|\Sigenv^{-1/2} \bhatw\|$. Write $\bhatv = \alpha \bstv + \sqrt{1-\alpha^2}\bv$, where $\bv \perp \bstv$. Observe that if $\alpha \le 0$, then $\|\bhatv - \bstv\|^2 \ge (1-\alpha)^2 + 1-\alpha^2 = 2 - 2 \alpha \ge 2$. So that $\Renv(\what) \le 1 \le c\|\bhatv - \bstv\|$ holds for any constant $c \ge 1/\sqrt{2}$.

Now consider when $\alpha \ge 0$. Finally, set $z_1 := \langle \bz,\bstv\rangle$, and $z_2 = \langle \bz,\bv \rangle$. Then,
\begin{align*}
\Renv(\what) &:= \Pr_{\env}[\sign(\langle \bx, \bhatw \rangle) \ne  \sign(\bx,\bstw)]\\
&= \Pr_{\env}[\sign(\langle \bz, \bhatv \rangle) \ne  \sign(\bz,\bstv)]\\
&=  \Pr_{\env}[\sign(z_1) \ne \sign (\alpha z_1  + \sqrt{1-\alpha^2}z_2 )] \\
&\overset{(i)}{=}  \frac{1}{2}\Pr_{\env}[\alpha |z_1|  \le \sqrt{1-\alpha^2}|z_2|]\\
&=  \frac{1}{2}\Pr_{\env}[ |z_1/z_2|  \le \frac{\sqrt{1-\alpha^2}}{\alpha} ]\\
&\overset{(ii)}{=}  \Pr_{\env}\left[ 0 \le z_1/z_2  \le \frac{\sqrt{1-\alpha^2}}{\alpha} \right],
\end{align*}
where in $(i)$ and $(ii)$, we used that $z_2 \mid z_1$ is symmetric around the origin. Notice that $z_1/z_2$ is a Cauchy-random variable, and $\alpha \ge 0$. Writing $\alpha = \cos(\theta)$, we have $\frac{\alpha}{\sqrt{1-\alpha^2}} = \tan(\theta)$. 
\begin{align*}
\Renv(\what) = \frac{1}{\pi}\left(\arctan(\tan(\theta)) - \arctan(0)\right) = \frac{1}{\pi}( \theta) = \frac{\theta}{2\pi}. 
\end{align*}
Next, observe that 
\begin{align*}
\theta = \arccos( \langle \bstv, \bhatv \rangle ) = \langle \bstv, \bhatv \rangle = \arccos(1 - \|\bstv - \bhatv\|^2)
\end{align*}
We now use that $\arccos(1-x) \le c\sqrt{x}$ for a universal $c$, which yields
\begin{align*}
\Renv(\what) &\le \frac{c}{2\pi} \|\bstv - \bhatv\| \\
&= \frac{2}{2\pi}  \left\| \frac{\Sigenv^{-1/2}\bwst}{\|\Sigenv^{-1/2}\bwst\|} - \frac{\Sigenv^{-1/2}\bhatw}{\|\Sigenv^{-1/2}\bhatw\|}\right\|\\
&\le \frac{c}{\pi \|\Sigenv^{-1/2}\bwst\|} \cdot \min_{\gamma \ge 0}\left\|\Sigenv^{-1/2}\bstw - \gamma \Sigenv^{-1/2}\bhatw\right\|,
\end{align*}
which concludes the proof. 

\end{proof}

\newcommand{\OPT}{\mathrm{OPT}}
\begin{lemma}\label{lem:renomalize} Let $\bw,\bv$ be two nonzero vectors. Then,
\begin{align*}
\left\|\bw/\|\bw\| - \bv/\|\bv\|\right\| \le 2 \min_{\gamma \ge 0}\|\bw\|^{-1} \cdot \|\bw - \gamma \bv\|. 
\end{align*}
\end{lemma}
\begin{proof} Lets assume $\bw,\bv$ are unit vectors. By rotating, we may assume without loss of generality that $\bw =\be_1$. Set $\bv = \alpha e_1 + \beta e_2$. Then.
\begin{align*}
\OPT := \min_{\gamma \ge 0} \|\bw - \gamma \bv\|^2 &= \min_{\gamma} (1-\gamma \alpha)^2 + (\beta \gamma)^2 = 1-2 \gamma \alpha + \gamma^2 (\alpha^2 + \beta)^2 = 1 - 2\alpha \gamma + \gamma^2 
\end{align*}
On the other hand,
\begin{align*}
\Delta := \|\bw - \bv\|^2 = 1 - 2\alpha + 1 = 2(1-\alpha)
\end{align*}
We consider two cases. If $\alpha \ge 0$, the $\OPT$ is attained at $\gamma = \alpha$, giving a miniimal value of $1-\alpha^2 = (1-\alpha)(1+\alpha) \ge \Delta/2$. On the other hand, if $\alpha \le 0$, then $\OPT = 1 \ge \Delta/4$.  Hence, for unit vectors $\bv$, we conclude
\begin{align*}
 \min_{\gamma \ge 0} \|\bw - \gamma \bv\|^2 \ge \frac{1}{4}\|\bw - \bv\|^2,
\end{align*}
So that, by rearranging, we have that $\|\bw - \bv\| \le 2\min_{\gamma \ge 0}\|\bw - \gamma \bv\|$.

Now, in the general case, we conclude that
\begin{align*}
\left\|\bw/\|\bw\| - \bv/\|\bv\|\right\| &\le 2 \min_{\gamma \ge 0} \left\|\bw/\|\bw\| - \gamma \bv/\|\bv\|\right\|\\
&= 2 \min_{\gamma \ge 0} \left\|\bw/\|\bw\| - \gamma \bv\right\|\\
&= 2 \min_{\gamma \ge 0} \|\bw\|^{-1} \cdot \left\|\bw - \gamma \bv\right\|
\end{align*}

\end{proof}



\begin{proof}[Proof of \Cref{thm:dist_shift_class}]
Using the above lemma ??, we have
\begin{align*}
\Renv(\what) &\le c \|\Sigenv^{-1/2} \bstw\|^{-1} \cdot \min_{\gamma \ge 0}\|\Sigenv^{-1/2}(\bstw - \gamma \bhatw)\|\\
&=  c \|\Sigenv^{-\half} \bstw\|^{-1} \cdot \min_{\gamma \ge 0}\|\Sigenv^{-\half}\Sigzero^{\half}(\Sigzero^{-\half}\bstw - \gamma \bP_{\envzero}\Sigzero^{-\half}\bhatw - \gamma(\eye_d - \bP_{\envzero}) \Sigzero^{-\half}\bhatw\|\\
&=  c \|\Sigenv^{-\half} \bstw\|^{-1} \cdot \min_{\gamma \ge 0}\|\Sigenv^{-\half}\Sigzero^{\half}(\Sigzero^{-\half}\bstw - \gamma \frac{\Sigzero^{-\half}\bstw \cdot (\bstw)^\top \Sigzero^{-1}\bhatw }{\|\Sigzero^{-1/2}\bstw\|^2}- \gamma\bhatw^{\perp}\|.
\end{align*}
Selecting $\gamma = \gamma_{\star} := \frac{\|\Sigzero^{-1/2}\bstw\|^2}{(\bstw)^\top \Sigzero^{-1}\bhatw }$, we find
\begin{align*}
\Renv(\what) \le \frac{c \gamma_{\star}}{\|\Sigenv^{-\half} \bstw\|} \|\Sigenv^{-\half}\Sigzero^{\half} \cdot \bhatw^{\perp} \|.
\end{align*}
Observing that $\bhatw^\perp$ lies in the co-kernel of $(\eye_d - \bP_{\envzero})$, we have 
\begin{align*}
\Renv(\what) &\le \frac{c \gamma_{\star}}{\|\Sigenv^{-\half} \bstw\|} \|\Sigenv^{-\half}\Sigzero^{\half}(\eye_d - \bP_{\envzero}) \cdot \bhatw^{\perp} \|\\
&\le \frac{c \gamma_{\star}}{\|\Sigenv^{-\half} \bstw\|} \| (\bhatw^{\perp})^\top(\eye_d - \bP_{\envzero})(\Sigzero^{\half}\Sigenv^{-1}\Sigzero^{\half})(\eye_d - \bP_{\envzero}) \cdot \bhatw^{\perp} \|^{1/2}
\end{align*}
Since $\bhatw^{\perp}$ is uniform on the sphere, a Hanson-Wright inequality shows that the above concentrates around
\begin{align*}
\frac{c \gamma_{\star}}{\|\Sigenv^{-\half} \bstw\|} \cdot \trace((\eye_d - \bP_{\envzero})(\Sigzero^{\half}\Sigenv^{-1}\Sigzero^{\half})(\eye_d - \bP_{\envzero}))^{1/2}  &= \frac{c \gamma_{\star}}{\|\Sigenv^{-\half} \bstw\|} \sqrt{\trace(\Sigenv^{-1}\Sigzero^{\half}(\eye_d - \bP_{\envzero})\Sigzero^{\half} )}
\end{align*}
\end{proof}

==> body/experiment_ideas.tex <==
%!TEX root = ../main.tex
\newpage
\section{Experiment \& Example Ideas}

\subsection{Baselines:}
We consider a class of methods $\cM := \{M\}$
\begin{enumerate}
	\item Linear Regression Classifier
	\item SVM
	\item Kernel SVM
	\item MLP
	\item Conv Net
	\item Others?
\end{enumerate}

\begin{hypoth} Consider a predictor which makes an assessment
\end{hypoth}
\subsection{Dataset 1: The Celeb-A Dataset}
This dataset is given in \url{https://mmlab.ie.cuhk.edu.hk/projects/CelebA.html}. This has multiple images, let us call them $\bw$, each with a binary vector of attributes $\mathbf{a} \in \{0,1\}^{k}$. 
Let us denote the true correspondence between then $\mathbf{a} = \phi_{\star}(\bw)$. 

\begin{definition} For each attribute $i \in [k]$ and method $M \in \cM$ and $\rho \in (0,1)$, set $R_{M,i,\rho}$ to be the error of predicting attribute $i$ on a standard test-train split of the ``aligned-and cropped'' images, where $\rho$ is tuned so that on the test and train, we ensure there are $\rho$-fraction positives and $1-\rho$-fraction negatives. We aim to study how predictive $R_{M,i,\rho}$ is of distribution shifts.
\end{definition}

\begin{itemize}
	\item Experiment 1a: How does $R_{M,i,\rho}$ predict performance on prediction on the ``in-the-wild dataset''? Here, we should normalize the ``in-the-wild'' dataset to have the same attribute proportions dictated by $\rho$. The same can be done with shifts by location.
	\item Experiment 1b: For each attribute $i$, how do shifts in the attribute proportions of attributes $j \ne i$ affect performance on the attribute $i$? Here, we should test both the case when we, shift proportions in attribute $j$ to maintain fixed proportions of attribute $i$, and when we do not
	\item Experiment 1c: Consider a logical predicate $\chi(\ba)$, e.g. $\chi_{i,j}(\ba) = \ba_i \mathrm{XOR} \ba_j$. Are $R_{M,i,\rho}$ and $R_{M,j,\rho}$ predictive of performance when the proportions of $\ba_i$ or $\ba_j$ are changed. 
\end{itemize}

\subsection{Dataset 2: Civil-Comments WILDs}
We study the Civil-Comments WILDs dataset in 
\url{https://authors.library.caltech.edu/111571/2/2012.07421.pdf}. Here, let $\bw$ denotes a string of text, with binary attribute vector $\ba \in \{0,1\}^8$ and label $\bz \in \{0,1\}$ denoting whether the comment is labeled toxic or not. Let $p$ denote the proportion of $\bz = 1$ in the same data and  $R_{M,i,\rho}$ denote the error in \emph{predicting } attributed $\ba_i$ from the text using method $M$, when $\ba_i = 1$ is balanced to have proporition $\rho$. 
\begin{itemize}
	\item Experiment 2a: Does $R_{M,i,\rho}$ predict the error of method $M$ on prediction under subpoulation shift of attribute $i$?
	\item Experiment 2b: Does $R_{M,i,\rho}$ predict the error of method $M$ on prediction under subpoulation shift of attribute $i$, when the shift is corrected to ensure that the labels $\bz$ exhibit the same class balance given by the fraction $p$ ?
\end{itemize}
\subsection{Experiment 3: Numerical Simulation}
\mscomment{think of simulations which verify the theoretical findings in this work}
We consider precisely the setting in this work. Fix normal distributions 
\begin{align*}
\cN_{x,1},\dots,\cN_{x,k}, \quad \cN_{y,1},\dots,\cN_{y,k},
\end{align*}
where 
\begin{align*}
\cN_{x,\ell} \sim \cN(\mu_{x,\ell}, \Sigma_{x,\ell}), \quad \cN_{y,\ell} \sim \cN(\mu_{y,\ell}, \Sigma_{y,\ell}),
\end{align*}
and where $\mu_{x,\ell} \sim \cS^{d_x - 1}$, $\mu_{y,\ell} \sim \cS^{d_y - 1}$, and $\Sigma_{x,i}$ and $\Sigma_{y,i}$ are drawn uniformly on the set of covariance matrices with trace $1$. For vectors $p, q \in \Delta^{k-1}$ on the $k$-simplex, define the mixture distributions
\begin{align*}
\cD_{x,p} := \sum_{\ell} p_\ell \cN_{x,\ell} \quad \cD_{y,q} := \sum_{\ell} q_\ell \cN_{q,\ell},
\end{align*} 
and define the product distribution
\begin{align*}
\cD_{p, q} := \cD_{x,p} \otimes \cD_{y,q}. 
\end{align*}
For function class $\cF_i$ and $\cG_j$, fix some ground truth $f_{\star,i} \in \cF_i$ and $g_{\star,i} \in \cG_j$
let $R^x_{i,\sigma}$ denote the error of predicting $f_{\star,i}$ with noise $\sigma > 0$ under $\bx \sim \cD_{x,p}$ and $R^y_{j,\sigma}$ denote the error of predicting $g_{\star,k}$ with noise $\sigma > 0$ under $\by \sim \cD_{y,q}$, where $p,q = 1/K$.  
\begin{itemize}
	\item Experiment 3a: How does $R^x_{i,\sigma}$ and $R^y_{j,\sigma}$ predict robustness to changing $p$ and $q$ across different pairs of $i$ and $j$? When $f+g$ are trained \emph{jointly?}
	\item Experiment 3b: How does this compare to the behavior when $f$ and $g$ are trained \emph{separetly}? (Double ML)
\end{itemize}

\subsection{Experiment 4: Procgen Maze}
% Color v.s. Maze \mscomment{to do}
\aacomment{
We study procgen mazes, wherein an agent is put in a maze and it needs to find its way to the goal location. The agent gets a top down view of the maze. The goal is to learn a policy $\pi_\theta(a|s)$ that allows agent to solve any maze $M \in P(M)$. Here, $a$ represents the action and $s$ contains the top down image of the agent and the goal in maze $M$. A maze $M$ has 2 properties: (i) a layout $L$ and (ii) a texture $T$. Furthermore, $P(M) = P(L)P(T)$ where $P(L)=\text{Categorical}(\{L_i\}_{i=1}^{N_L}; \theta_L)$ and $P(T)=\text{Categorical}(\{T_i\}_{i=1}^{N_T}; \theta_T)$. Let's say we sampled $M_{\text{train}} = \{M_i \sim P(M)\}$ and $M_{\text{test}} = \{M_i \sim P(M)\}$. We train a classifier $f_\phi$ on $M_{\text{train}}$ such that $f_\phi(M) \approx P(L,T|M)$ tries to predict the layout id and the texture id from map $M$ (represented as an image). We assume that the empirical distribution of $L$ and $T$ in $M_{\text{train}}$ and $M_{\text{test}}$ also remain as $\theta_L$ and $\theta_T$ respectively. Let $R_{f_\phi, L, \theta_L}$ be the prediction error of the classifier $f_\phi$ for layout on $M_{\text{test}}$. Similarly, let $R_{f_\phi, T, \theta_T}$ be the prediction error of the classifier $f_\phi$ for texture on $M_{\text{test}}$.
\begin{itemize}
	\item Experiment 4a: Does $R_{f_\phi, T, \theta_T}$ predict the success rate of the policy $\pi_\theta$ when there's a distribution shift in texture (i.e. $T \sim Q(T)=\text{Categorical}(\{T_i\}_{i=1}^{N_T}; \bar{\theta}_T)$)?
    \item Experiment 4b: Does $R_{f_\phi, L, \theta_L}$ predict the success rate of the policy $\pi_\theta$ when there's a distribution shift in layout (i.e. $L \sim Q(L)=\text{Categorical}(\{L_i\}_{i=1}^{N_L}; \bar{\theta}_L)$)?
\end{itemize}
}

\subsection{Experiment 5: Quadruped Reaching}
% To one-step dynamics prediction predict distribution shift with an attribute?
\aacomment{
We study quadruped reaching, where a quadruped agent needs to navigate to a fixed goal location. The state $s$ of the agent is given by joint angles and the $(x,y)$ location of its center of mass in the global frame. The MDP $\mathcal{M}$ (that defines the reaching task) is parameterized by mass $m$ of the quadruped and the length of its legs $l$. The goal is to learn a policy $\pi_\theta(a|s,m,l)$ that allows agent to solve the navigation task for any MDP $\mathcal{M} \sim P(\mathcal{M})$. Here, $P(\mathcal{M})=P(m)P(l)$ where $P(m)=\mathcal{N}(\mu_m, \Sigma_m)$ and $P(l)=\mathcal{N}(\mu_l, \Sigma_l)$. Let's say we sampled $m_{\text{train}} = \{m_i \sim P(m)\}$, $m_{\text{test}} = \{m_i \sim P(m)\}$, $l_{\text{train}} = \{l_i \sim P(l)\}$, and  $l_{\text{test}} = \{l_i \sim P(l)\}$. We train a dynamics model $p_\phi(s'|s,a,m,l)$ on $\mathcal{M}_{\text{train}} = m_{\text{train}} \times l_{\text{train}}$. Let $R_{p_\phi,m,(\mu_m, \Sigma_m)}$ be the average prediction error of the dynamics model on $m_{\text{test}}\times l_{\text{train}}$. Similarly, let $R_{p_\phi,l,(\mu_l, \Sigma_l)}$ be the average prediction error of the dynamics model on $m_{\text{train}}\times l_{\text{test}}$.
\begin{itemize}
	\item Experiment 5a: Does $R_{p_\phi,m,(\mu_m, \Sigma_m)}$ predict the success rate of the policy $\pi_\theta$ when there's a distribution shift in quadruped's mass $m$ (i.e. $m \sim Q(m)=\mathcal{N}(\bar{\mu}_m, \bar{\Sigma}_m)$)?
    \item Experiment 5b: Does $R_{p_\phi,l,(\mu_l, \Sigma_l)}$ predict the success rate of the policy $\pi_\theta$ when there's a distribution shift in quadruped leg's length $l$ (i.e. $l \sim Q(l)=\mathcal{N}(\bar{\mu}_l, \bar{\Sigma}_l)$)?
\end{itemize}
}

==> body/old_stuff.tex <==

\begin{comment}

\begin{lemma}
\end{lemma}
\begin{proof}  Let $h$ be a family of uniformly bounded functions with $|h|\le B$. $\sup_{h \in \cH(r)}\Var[h(\bw)^2] \le r^2$,  \citet[Theorem 2.1]{bartlett2005local},  with probability $1 - \delta$, 
\begin{align*}
\inf_{h \in \cH}\frac{1}{n}\sum_{n=1}^n \Exp[h] - h(\bw_i)  &\lesssim \Radenp(\cH(r)) + r\sqrt{\frac{ \log(1/\delta)}{n}} + \frac{B^2\log(1/\delta)}{n}\\
&\lesssim \Radenp(\cH(r)) + r^2 + \frac{B^2\log(1/\delta)}{n},
\end{align*}
where in the second line, we use AM-GM and $B \ge 1$. Next, we consider
\begin{align*}
2\Radenp(\cH(r)) - \frac{r^2}{2} &= 2\Exp_{\bw_{1:n}}\left[\sup_{h \in \cH(r)}\Exp_{\epsvar_{1:n}}\left[\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right]\right] - \frac{r^2}{2}\\
&= \Exp_{\bw_{1:n}}\left[\sup_{h \in \cH(r)}\Exp_{\epsvar_{1:n}}\left[\frac{2}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right] - \frac{r^2}{2}\right] \\
&\le \Exp_{\bw_{1:n}}\left[\sup_{h \in \cH(r)}\Exp_{\epsvar_{1:n}}\left[\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right] - \frac{1}{2}\Exp[h(\bw_i)^2]\right] \tag{Definition of $\cH(r)$}\\
%&\le \Exp_{\bw_{1:n}}\left[\sup_{h \in \c}\Exp_{\epsvar_{1:n}}\left[\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right] - \frac{1}{2}\Exp[h(\bw_i)^2]\right] \tag{ $\cH(r)\subset$}\\
%&\le \Exp_{\bw_{1:n}}\Exp_{\bw_{1:n}}\left[\sup_{h \in \cH(r)}\Exp_{\epsvar_{1:n}}\left[\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right] - \frac{1}{2}\Exp[h(\bw_i)^2]\right] \tag{Jensen's i}\\
%&= 2\Exp_{\bw_{1:n}}\left[\sup_{h \in \cH(r)}\Exp_{\epsvar_{1:n}}\left[\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i)\right] - \frac{r^2}{2}
\end{align*}
\end{proof}

\begin{lemma}[Uniform Convergence, Theorem 2.1 n \cite{bartlett2005local}]\label{lem:rad_uniform_convergence} Let $h$ be a family of uniformly bounded functions with $|h|\le B$ and $\sup_{h \in \cH}\Var[h^2] \le \nu^2$. Then, with probability at least $1 - \delta$, 
\begin{align*}
\inf_{h \in \cH}\frac{1}{n}\sum_{n=1}^n \Exp[h] - h(\bw_i)  \le \left(6\Radenp(\cH) + \sqrt{\frac{2\nu^2 \log(1/\delta)}{n}} + \frac{11 B^2\log(1/\delta)}{n}\right)\\
\le \left(6\Radenp(\cH) + \sqrt{\frac{2\nu^2 \log(1/\delta)}{n}} + \frac{11 B^2\log(1/\delta)}{n}\right)
\end{align*}
In particular, if $\cH = \cH(r)$ for some $r$, then the above holds for $\sigma^2 = r^2$.
\end{lemma}


\newcommand{\rquad}{r_{\mathrm{quad}}}
\begin{lemma}[Quadratic Bounds]\label{lem:quad_lb} Let $B \ge 1$, and $\cH$ be a star-shaped function class from $\cW \to \R$ such that $\sup_{w \in \cW}|h(w)| \le B$, and let $\bw_1,\dots,\bw_n \iidsim \Pr$. For a sufficiently large universal constant $c \ge 1$, define
\begin{align}
\rquad(\cH,\delta)^2 := c B^2 \delnst(\cH )^2 + \frac{ B^2\log(1/\delta)}{n}  \label{eq:rnot_def} 
\end{align}
with probability $1-\delta$, the following holds that for all $h \in \cH$ 
\begin{align}
\frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 \ge \Exp[h(\bw)^2] - \frac{\rquad(\cH,\delta)^2}{4} \label{eq:some_lb_rnot_quad}
\end{align}
By increasing the constant $c$ above if necessary, it also holds that for any $r \ge \rquad(\cH,\delta)$ and another universal constant $c'$ that with probability $1-\delta$, 
\begin{align*}
\sup_{h \in \cH(r)} \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 \le c' r^2
\end{align*}
\end{lemma}
\begin{proof} We prove the first bound as the second is analogous. Adopt the shorthand $\rquad = \rquad(\cH,\delta)$. We first establish a lower bound over $\cH(\rquad)$, and then use the star-shaped property to extend to the entire class $\cH$. For $\cH(\rquad)$, using \Cref{lem:rad_uniform_convergence} and setting $\nu := \sup_{h \in  H(\rquad)}\Var[h]$ yields that with probability $1 - \delta$,
\begin{align*}
\inf_{h \in \cH(\rquad)} \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 - \Exp[h(\bw_i)^2] \ge -\left(6\Radenp( \cH(\rquad)) + \nu\sqrt{\frac{2 \log(1/\delta)}{n}} + \frac{11 B^2\log(1/\delta)}{n}\right).
\end{align*}
By assumption $|h| \le B$ for $h \in  \cH$; thus, we may take $\nu \le \rquad B$. Moreover, using Lipschitz contraction that the fact $t \mapsto t^2$ is  $2B$-Lipschitz on $[-B,B]$, we have that with probability $1- \delta$,
\begin{multline}
\inf_{h \in \cH(\rquad)} \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 - \Exp[h(\bw_i)^2] \\
\le -\left(12B\Radenp(\cH(\rquad)) + \rquad B\sqrt{\frac{2 \log(1/\delta)}{n}} + \frac{11 B^2\log(1/\delta)}{n} \right) \label{eq:some_Hquad_eq}
\end{multline}
In particular, if $\rquad$ satisfies
\begin{align}
12B\Raden(\cH(\rquad)) + \rquad B\sqrt{\frac{2 \log(1/\delta)}{n}} + \frac{11 B^2\log(1/\delta)}{n} \le \frac{1}{4} \rquad^2  \label{eq:not_wts},
\end{align}
it holds that 
\begin{align}
\forall h \in \cH(\rquad), \quad \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 \ge \Exp[h(\bw)^2] - \frac{1}{4}\rquad^2   \label{eq:lb_on_Hnotr}
\end{align}
This establishes \Cref{eq:some_lb_rnot_quad} restricted to $h \in \cH(\rquad)$. To conclude,  suppose $h \in \cH \setminus \cH(\rquad)$, so that $\Exp[h(\bw)^2] \ge \rquad^2$. Then, setting $\alpha = \rquad/\sqrt{\Exp[h(\bw)^2]}$  and $\alpha h \in \cH(\rquad)$, and thus
\begin{align*}
\alpha^2 \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 \ge \alpha^2\Exp[h(\bw)^2]  - \frac{1}{4}\rquad^2 = \frac{3}{4}\rquad^2 
\end{align*}
Hence, as $\Exp[h(\bw)^2] \ge \rquad^2$, we have
\begin{align*}
 \frac{1}{n}\sum_{i=1}^n h(\bw_i)^2 \ge \frac{3}{4}\rquad^2/\alpha^2 = \frac{3}{4}\Exp[h(\bw)^2] = \Exp[h(\bw)^2] - \frac{1}{4}\Exp[h(\bw)^2] \ge  \Exp[h(\bw)^2] - \frac{1}{4}\rquad^2. 
\end{align*}
To conclude, it suffices to show that $\rquad$ satisfies \Cref{eq:not_wts}. To select $\rquad = r $, where $c$ is a universal constant and $r$ satisfies
\begin{align*}
r\ge  cB \Raden(\cH(r)), \quad r^2 \ge  c12 r\sqrt{\frac{ \log(1/\delta)}{n}}, \quad cr^2 \ge \frac{ B^2\log(1/\delta)}{n}.
\end{align*} 
It is clear $\rquad$ in  \Cref{eq:rnot_def}  can be made to satisfy the second and third inequality by picking constants appropriately. For the first, we observe that 
\begin{align*}
cB\Radenp(\cH(r)) - \frac{1}{2}r^2 &= cB\Exp_{\bw_{1:n}}\Exp_{\epsvar_{1:n}}\sup_{h \in \cH(r)}\frac{1}{n}\sum_{i=1}^n h(\bw_i) - \frac{1}{2}r^2\\
&\le cB\Exp_{\bw_{1:n}}\Exp_{\epsvar_{1:n}}\sup_{h \in \cH(r)}\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i) - \frac{1}{2}\Exp[h(\bw_i)^2] \tag{definition of $\cH(r)$}\\
&\le cB\Exp_{\bw_{1:n}}\Exp_{\epsvar_{1:n}}\sup_{h \in }\frac{1}{n}\sum_{i=1}^n \epsvar_i h(\bw_i) - \frac{1}{2}\Exp[h(\bw_i)^2] \tag{ $\cH(r) \subset \cH$}
\end{align*}
Arguing as in the proof of \Cref{lem:gauss_offset} and using $B \ge 1$ and \Cref{lem:star_shaped} where appropriate, we see that
\begin{align*}
\sup_{r} 12B\Radenp(\cH(r)) - \frac{1}{2}r^2 \lesssim B^2\updelta_{n,\star}(\cH)^2 + \frac{B^2\log(1/\delta)}{n}. 
\end{align*}
Hence, by selecting $r^2 \gtrsim B^2\updelta_{n,\star}(\cH)^2 + \frac{B^2\log(1/\delta)}{n}$, the proof follows. 
\end{proof}

\end{comment}

\begin{lemma}[Rademacher Lipschitz Contraction with Offset]\label{lem:offset_contraction} Let $\bbV \subset \R^n$, and let $\phi: \R \to \R$ be $L$-Lipschitz, and $\tilde \phi : \R \to \R$ be arbitrary. 
\begin{align*}
\Exp_{\epsvar_{1:n}}\left[\sup_{v \in \bbV} \sum_{i=1}^n \epsvar_i \phi (v_i)   - \tilde{\phi}(v_i)\right] \le \Exp_{\epsvar_{1:n}}\left[\sup_{v \in \bbV} \sum_{i=1}^n L\epsvar_i  v_i   - \tilde{\phi}(v_i)\right]
\end{align*}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:offset_contraction} ]  The proof follows along the same lines as that of the standard contraction inequality for Rademacher complexity (e.g. \citet[Lemma 29]{rakhlinnotes}). Define the partial sum $S_k(v,\bepsilon_{1:k}) := \sum_{i=1}^k \epsvar_i \phi (v_i)   -  \sum_{j=1}^n\tilde{\phi}(v_j)$ (which contain the all $n$ offset terms). Then, 
\begin{align*}
\Exp_{\epsvar_{1:n}}\left[\sup_{v \in \bbV} \sum_{i=1}^n \epsvar_i \phi (v_i)   - \tilde{\phi}(v_i)\right] &= \Exp_{\epsvar_{1:n}}\left[\sup_{v \in \bbV} S_{n-1}(v,\bepsilon_{1:n-1})+ \epsvar_n \phi (v_n) \right]\\
\end{align*}
Condition on $\epsvar_{1:n-1}$, and write $S_{n-1}(v,\bepsilon_{1:n-1}) = S_{n-1}(v)$ for shorthand. Then, 
\begin{align*}
& \Exp_{\epsvar_n}\left[\sup_{v \in \bbV}S_{n-1}(v)+ \epsvar_n \phi(v_n)\right]\\
%
&= \frac{1}{2}\sup_{v \in \bbV}\left[S_{n-1}(v)+  \phi(v_n)\right] + \frac{1}{2}\sup_{v \in \bbV}\left[S_{n-1}(v)-  \phi(v_n)\right] \tag{computing the expectation}\\
%
&= \frac{1}{2}\sup_{v \in \bbV}\left[S_{n-1}(v)+  \phi(v_n)\right] + \frac{1}{2}\sup_{v' \in \bbV}\left[S_{n-1}(v')-  \phi(v_n')\right]\\
&= \frac{1}{2}\sup_{v,v' \in \bbV}\left[S_{n-1}(v)+  S_{n-1}(v') + \phi(v_n) -  \phi(v_n')\right]\\
&\le \frac{1}{2}\sup_{v,v' \in \bbV}\left[S_{n-1}(v)+  S_{n-1}(v') + |\phi(v_n) -  \phi(v_n')|\right] \\
&\le \frac{1}{2}\sup_{v,v' \in \bbV}\left[S_{n-1}(v)+  S_{n-1}(v') + L|v_n -  v_n'|\right] \tag{Lipschitz property}\\
&\overset{(i)}{=}  \frac{1}{2}\sup_{v,v' \in \bbV}\left[S_{n-1}(v)+  S_{n-1}(v') + L(v_n -  v_n')\right] \\
&=  \Exp_{\epsvar_n}\left[\sup_{v \in \bbV}S_{n-1}(v)+ \epsvar_n  L v_n\right].
\end{align*}


\begin{proof} We compute
\begin{align*}
&\Exp_{\bw_{1:n}}\left[\sup_{h \in \cH} \|h(\bw_{1:n})\|_{2,n}^2 - (1+\gamma)\Exp[h(\bw)^2]\right]\\
 &= \Exp_{\bw_{1:n}}\left[\sup_{h \in \cH} \|h(\bw_{1:n})\|_{2,n}^2 - (1+\gamma)\Exp_{\bw_{1:n}'}\|h(\bw_{1:n}')\|_{2,n}^2\right]  \\
&\le \Exp_{\bw_{1:n},\bw_{1:n'}}\left[\sup_{h \in \cH} \|h(\bw_{1:n})\|_{2,n}^2 - (1+\gamma)\|h(\bw_{1:n}')\|_{2,n}^2\right] \tag{swapping $\Exp$ and $\sup$}  \\
&= \Exp_{\bw_{1:n},\bw_{1:n}'}\left[\sup_{h \in \cH} (1+\frac{\gamma}{2})\left(\|h(\bw_{1:n})\|_{2,n}^2 -\|h(\bw_{1:n}')\|_{2,n}^2\right)  - \frac{\gamma}{2}\left(\|h(\bw_{1:n})\|_{2,n}^2 +\|h(\bw_{1:n}')\|_{2,n}^2\right) \right]\\
&= \frac{1}{n}\Exp_{\bw_{1:n},\bw_{1:n}'}\left[\sup_{h \in \cH} \sum_{i=1}^n (1+\frac{\gamma}{2})\left(h(\bw_i)^2 - h(\bw_{i}')^2\right)   - \frac{\gamma}{2}\left(h(\bw_i)^2\ +h(\bw_{i}')^2\right) \right]\\
&= \frac{1}{n}\Exp_{\bw_{1:n},\bw_{1:n}'}\Exp_{\epsvar_{1:n}}\left[\sup_{h \in \cH} \sum_{i=1}^n (1+\frac{\gamma}{2})\epsvar_i\left(h(\bw_i)^2 - h(\bw_{i}')^2\right)   - \frac{\gamma}{2}\left(h(\bw_i)^2\ +h(\bw_{i}')^2\right) \right]\\
&\le \frac{2}{n}\Exp_{\bw_{1:n}}\Exp_{\epsvar_{1:n}}\left[\sup_{h \in \cH} \sum_{i=1}^n (1+\frac{\gamma}{2})\epsvar_ih(\bw_i)^2   - \frac{\gamma}{2} h(\bw_i)^2\right] \tag{Standard symmetrization}\\
&\le \frac{2}{n}\Exp_{\bw_{1:n}}\Exp_{\epsvar_{1:n}}\left[\sup_{h \in \cH} \sum_{i=1}^n (2+\gamma)B\epsvar_ih(\bw_i)   - \frac{\gamma}{2} h(\bw_i)^2\right], 
\end{align*}
where in the last inequality we use \Cref{lem:offset_contraction} with $\phi(z) = (1+\frac{\gamma}{2})z^2$, $\tilde{\phi}(z) = \frac{\gamma}{2}z^2$, and notice that $\phi(z)$ is $2B\cdot(1+\frac{\gamma}{2}) = B(2+\gamma)$-Lipschitz for $|z| \le B$.
\end{proof}
Here, in $(i)$, we use symmetry with respect to $v,v'$: indeed, if $\bar v,\bar v'$ attain (for any given $\eta > 0$) $S_{n-1}(\bar v)+  S_{n-1}(\bar v') + L|\bar v_n -  \bar v_n'| \ge - \eta + \sup_{v,v' \in \bbV}S_{n-1}(v)+  S_{n-1}(v') + L|v_n -  v_n'|$, then either $\bar v_n \ge \bar v_n'$, or else one can swap $\bar v$ and $\bar v'$ to ensure that this is the case. The proof now follows by iteractively applying the above argument 
\end{proof}

==> body/sum_regressors.tex <==
%!TEX root = ../main.tex



\section{Results 2}

\subsection{Main Result}
\paragraph{Notation.} 



\mscomment{Remark that the prameter $\tau_2$ is redundant, but makes computations cleaner because logarithmics can be negative.}
Throughout, $C_p$ is an unspecified positive constant that depends on $p$.


\begin{restatable}[Tail Terms]{definition}{tailterms} Given $\cH \subset \{\cW \to \R\}$ and $q \in [1,\infty]$, define\label{defn:tailterms}
\begin{align*}
\Phingl[q](\cH) := \inf  B C_p\sqrt{\tau}\begin{cases} \sqrt{\log (c/B)} \cdot n^{-\frac{1}{2}} & p = 0\\
n^{-\frac{1}{2}} & p  < 2 \\
 n^{-\frac{1}{2}} \log n & p = 2 \\
  n^{-\frac{1}{p}} & p > 2 \\
\end{cases}, \quad \Phinloc[q](\cH) &:=  \inf C_p \begin{cases} \frac{\tau \log cn}{n} & p = 0 \\
(\frac{\tau}{n})^{\frac{2}{2+p}}  &  p \in (0,2)\\
\frac{\sqrt{\tau}\log n}{\sqrt{n}} & p = 2  \\
 \sqrt{\tau}(n)^{-\frac{1}{p}} & p > 2
\end{cases},
\end{align*}
where the infima is over all $(p,\tau)$ such that $\cH \in \entclass_{q}(p,\tau)$ or $(p = 0,\tau,c)$ such that $\cH \in \entclass_q(0,\tau,c)$. 
\end{restatable}
\begin{definition}[Key Classes] We define the following classes of interest 
\begin{align*}
\Fcent = (\{(f-\fst -\upbeta_f): f \in \cF\}), \quad \Gcent := (\{g - \gst + \upbeta_f: f \in \cF, g \in \cG\})
\end{align*}
\end{definition}


\mscomment{burn for $\cG$ is suficiently long that $\gamma^2$ necessary for conditional completeness}
\begin{theorem} Consider the case where $B^2 = 1$ for simplicity. Also, take $\gamma$ sufficiently small that $\dots$.  Then, with probability $1 - \delta$,
\begin{align*}
\Rzero[f] \lesssim (1+\sigma^2)\Phinloc[2](\Fcent) +   \Phingl[\infty](\Gcent)^2  + \frac{ (1+\sigma^2)\log(\log_2(n)/\delta)}{n}
\end{align*}
\end{theorem}


\begin{align*}
\Renv(f,g) = \nu_{x,y}\left( (1+\sigma^2)\Phinloc[2] +   \Phingl[\infty](\Gcent)^2 \right) + (1+\sigma^2)\nu_y \Phinloc[2](\cF + \cG) +  \frac{ \nu_{x,y}(B^2+\sigma^2)\log(\log_2(n)/\delta)}{n}
\end{align*}
\mscomment{no wins for parametric classes here}


\subsection{Faster Rates for Parametric Classes}




==> body/weak_conditional_completeness.tex <==
%!TEX root = ../main.tex

\section{Weak Conditional Completeness}


We will refer to \Cref{defn:conditional_complete} as \emph{strong} conditional completeness, distinguishing it from the following consider more lenient notion.
\begin{definition}[Weak Conditional Completness] Let $\psi: \R_{> 0}^2 \to \R_{\ge 0}$ and $\cG_{\upbeta} \subset \R^{\cY}$. We say 
\begin{itemize}
\item[(a)] $(\cF,\cG)$ satisfies $\psi$- weak conditional completeness if, for all $\gamma_1,\gamma_2 > 0$, and all 
\begin{align}
(f,g) \in \cF \times \cG \text{ s.t. } \Ezero[\Vzero[(f-\fst)(\xvar)]] \le \gamma_1,~ \Ezero[(g-\gst + \upbeta_f)(\yvar)^2] \le \gamma_2 \label{eq:weak_cond_comp},
\end{align} it holds that $\inf_{g_0 \in \cG} \Ezero[(g - g_0 + \upbeta_f)] \le \psi(\gamma_1,\gamma_2)$. 
\item[(b)]  $(\psi,\cG_{\upbeta})$-localized conditional completeness if for all $(f,g)$ and $(\gamma_1,\gamma_2)$ satisfying \Cref{eq:weak_cond_comp}, $g + \cG_{\upbeta} \subset \cG$, and  $\inf_{g_0 \in \cG_{\upbeta}} \Ezero[(g_0 + \upbeta_f)] \le \psi(\gamma_1,\gamma_2)$. 
\end{itemize}
\end{definition}
It is clear that any $(\cF,\cG)$ satisfy $\psi$-conditional completeness for the idenity function $\psi(\gamma_1,\gamma_2) = \gamma_2$. Moreover, $\gamma$- conditional completeness (in the strong sense) is precisely $\psi$-weak conditional completeness


==> preamble/reg_macros.tex <==
\newcommand{\lbr}{\lbrace}
\newcommand{\rbr}{\rbrace}

\newcommand{\ac}{{A_c}}
\newcommand{\bc}{{B_c}}
\newcommand{\cc}{{C_c}}
\newcommand{\dc}{{D_c}}

\newcommand{\cparams}{\ac,\bc,\cc,\dc}
\newcommand{\lmiparams}{X,Y,K,L,M,N}

%\newcommand{\transp}{^{\top}}
\newcommand{\invtransp}{^{-\top}}
\newcommand{\inv}{^{-1}}



\newcommand{\params}{\x}
\newcommand{\obj}{F}
\newcommand{\regf}{R}
\newcommand{\ccg}{\Sigma}
\newcommand{\robj}{G}

%\newcommand{\h}{h}
\newcommand{\dt}{\bar{T}}

\newcommand{\simt}{\mathcal{S}}
\newcommand{\shot}{\mathcal{S}_{\textup{hot}}}

\newcommand{\stpt}[1]{\bar{#1}}

\newcommand{\spoint}{\stpt{\params}}

%\newcommand{\xcl}{\mathcal{X}}
%
%\newcommand{\x}{\mathbf{x}}
%\newcommand{\y}{\mathbf{y}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\ytmp}{\bnu}

\newcommand{\dir}{\mathbf{d}}

\newcommand{\xc}{\bar{x}}

\newcommand{\miniheading}[1]{
	{\vspace{0.5em}
		\parindent0pt 
		\textbf{#1} \\
	}
}

\newcommand{\hot}{\textup{h.o.t}}
